A Structural Investigation of the Approximability of Polynomial-Time Problems

We initiate the systematic study of a recently introduced polynomial-time analogue of MaxSNP, which includes a large number of well-studied problems (including Nearest and Furthest Neighbor in the Hamming metric, Maximum Inner Product, optimization variants of $k$-XOR and Maximum $k$-Cover). Specifically, MaxSP$_k$ denotes the class of $O(m^k)$-time problems of the form $\max_{x_1,\dots, x_k} \#\{y:\phi(x_1,\dots,x_k,y)\}$ where $\phi$ is a quantifier-free first-order property and $m$ denotes the size of the relational structure. Assuming central hypotheses about clique detection in hypergraphs and MAX3SAT, we show that for any MaxSP$_k$ problem definable by a quantifier-free $m$-edge graph formula $\phi$, the best possible approximation guarantee in faster-than-exhaustive-search time $O(m^{k-\delta})$ falls into one of four categories: * optimizable to exactness in time $O(m^{k-\delta})$, * an (inefficient) approximation scheme, i.e., a $(1+\epsilon)$-approximation in time $O(m^{k-f(\epsilon)})$, * a (fixed) constant-factor approximation in time $O(m^{k-\delta})$, or * an $m^\epsilon$-approximation in time $O(m^{k-f(\epsilon)})$. We obtain an almost complete characterization of these regimes, for MaxSP$_k$ as well as for an analogously defined minimization class MinSP$_k$. As our main technical contribution, we rule out approximation schemes for a large class of problems admitting constant-factor approximations, under the Sparse MAX3SAT hypothesis posed by (Alman, Vassilevska Williams'20). As general trends for the problems we consider, we find: (1) Exact optimizability has a simple algebraic characterization, (2) only few maximization problems do not admit a constant-factor approximation; these do not even have a subpolynomial-factor approximation, and (3) constant-factor approximation of minimization problems is equivalent to deciding whether the optimum is equal to 0.

==> sections/baseline.tex <==
% !TEX root = ../paper.tex
\section{Baseline Algorithm} \label{sec:baseline}
There is a simple baseline algorithm solving any problem $\Max(\psi)$ or $\Min(\psi)$ in time $\Order(m^k)$. It is a straightforward adaption of the baseline algorithm for the decision setting in~\cite{GaoIKW18} to the optimization setting.

\begin{theorem}
Let $k \geq 1$ and let $\psi$ be an $\OptSP_k$ formula. Then $\Opt(\psi)$ can be solved exactly in time $\Order(m^k)$. In fact, we can compute the values $\Val(x_1, \dots, x_k)$ for all tuples $(x_1, \dots, x_k)$ in the same running time.
\end{theorem}
\begin{proof}
The proof is by induction on $k$. For $k = 1$, we obtain a linear-time improvement, and for larger $k$ we apply a downward self-reduction.
\begin{description}[leftmargin=0pt, itemsep=\topsep]
\item[Base case: \boldmath$k = 1$.] The problem is of the form $\psi = \opt_x \counting_y \phi(x, y)$. There are only three types of predicates: Unary predicates on $X$, unary predicates on $Y$ and binary predicates on $X \times Y$. In each case, we can alternatively think of a single multi-colored predicate. More specifically, suppose there are $a$ unary relations $R_1, \ldots, R_a$ on $X$. Then each object $x \in X$ is characterized by a \emph{color $\alpha(x) \in \{0, 1\}^a$}, where $\alpha_i = 1$ if and only if $R_i(x)$ is true. We similarly define colors $\beta(y)$ and $\gamma(x, y)$ for predicates on $Y$ and $X \times Y$. Moreover, we define $Y_\beta = \{ y \in Y : \beta(y) = \beta \}$. With this notation, we can rewrite the objective as
\begin{equation*}
  \OPT = \opt_{x \in X} \counting_{y \in Y} \phi(\alpha(x), \beta(y), \gamma(x, y)) = \opt_{x \in X} \sum_{\beta, \gamma} \phi(\alpha(x), \beta, \gamma) \mult \#\{ y \in Y_\beta : \gamma(x, y) = \gamma \},
\end{equation*}
where we abuse notation and interpret $\phi$ as a function which accepts colors as inputs. Let $C(x; \beta, \gamma) := \#\{ y \in Y_\beta : \gamma(x, y) = \gamma \}$. Suppose we have precomputed $C(x; \beta, \gamma)$ for all colors~$\beta, \gamma$ and for all $x \in X$. Then we can compute $\OPT$ in time $\Order(n) = \Order(m)$ by explicitly evaluating the above expression.

It remains to show that we can precompute all values $C(x; \beta, \gamma)$ in time $\Order(m)$. There are two cases: We say that a color $\gamma$ is \emph{black} if $\gamma = 0 = (0, \ldots, 0)$ and \emph{colorful} otherwise. First, if $\gamma$ is colorful, then we only have to consider pairs $(x, y)$ which occur positively in at least one binary predicate. Thus, there can be at most $\Order(m)$ such pairs and a single pass through the structure suffices to compute $C(x; \beta, \gamma)$. Second, if $\gamma$ is black, we compute $C(x; \beta, 0) = |Y_\beta| - \sum_{\gamma \neq 0} C(x; \beta, \gamma)$.

\item[Induction step: \boldmath$k \geq 2$.] Let $\psi = \opt_{x_1, \dots, x_k} \counting_y \phi(x_1, \dots, x_k, y)$. Our goal is to brute-force over all objects $x_1$. Fixing such an object $x_1$, we are left to optimize $\psi' = \opt_{x_2, \dots, x_k} \counting_y \phi'(x_2, \dots, x_k, y)$, for some propositional formula $\phi'$. We describe how to obtain $\phi'$ from $\phi$. Any predicate not including~$x_1$ remains untouched. Any predicate $R(x_1, x_{i_2}, \dots, x_{i_\ell})$ is replaced as follows: If $\ell = 1$ (that is, $R$ is unary), then $R(x_1)$ is replaced by the appropriate constant depending on whether $R(x_1)$ holds for the fixed object $x_1$. If $\ell > 1$, then we replace $R(x_1, x_{i_2}, \dots, x_{i_\ell})$ by $R'(x_{i_2}, \dots, x_{i_\ell})$ for a new relation $R'$. In the reduced instance, every $R$-record $(x_1, x_{i_2}, \dots, x_{i_\ell})$ is replaced by an $R'$-record $(x_{i_2}, \dots, x_{i_\ell})$ and all original entries not containing the fixed object $x_1$ are discarded. Notice that the total number of records can only decrease in this step. It is easy to verify that the above steps are correct, and that the objective does not change.

We inductively assume that $\Opt(\psi')$ can be solved exactly in time $\Order(m^{k-1})$. There are $n$ objects $x_1 \in X_1$, and for each such constructing the associated $\Opt(\psi')$ instance takes time $\Order(m)$. The total running time is $\Order(n m^{k-1}) = \Order(m^k)$. \qedhere
\end{description}
\end{proof}
